Combining Symbolic Expressions and Black-box Function Evaluations in Neural Programs

Neural programming involves training neural networks to learn programs, mathematics, or logic from data. Previous works have failed to achieve good generalization performance, especially on problems and programs with high complexity or on large domains. This is because they mostly rely either on black-box function evaluations that do not capture the structure of the program, or on detailed execution traces that are expensive to obtain, and hence the training data has poor coverage of the domain under consideration. We present a novel framework that utilizes black-box function evaluations, in conjunction with symbolic expressions that define relationships between the given functions. We employ tree LSTMs to incorporate the structure of the symbolic expression trees. We use tree encoding for numbers present in function evaluation data, based on their decimal representation. We present an evaluation benchmark for this task to demonstrate our proposed model combines symbolic reasoning and function evaluation in a fruitful manner, obtaining high accuracies in our experiments. Our framework generalizes significantly better to expressions of higher depth and is able to fill partial equations with valid completions.

==> app.tex <==
\appendix
\section*{Appendix}

\section{Details of Data Generation}

\paragraph{Set of Local Changes}
We first randomly select a node in the expression tree, followed by randomly selecting one of the following actions to make the local change to the equation at the selected node:
\begin{itemize}[noitemsep]
    \item \emph{ShrinkNode:} Replace the node, if it's not a leaf, with one of its children, chosen randomly.
    \item \emph{ReplaceNode:} Replace the symbol at the node (i.e. the terminal or the function) with another compatible one, chosen randomly.
    \item \emph{GrowNode:} Provide the node as input to another randomly drawn function $f$, which then replaces the node. If $f$ takes two inputs, the second input will be generated randomly from the set of terminals. 
    \item \emph{GrowSides:} If the selected node is an equality, either add or multiply both sides with a randomly drawn number, or take both sides to the power of a randomly drawn number.
\end{itemize}
%These local changes result in new identities that are valid expressions in the trigonometry grammar.


\cut{
\begin{table}[h]
\begin{tabular}{ccc}
\hline \\
Paper & Applications & data\\
\hline \\
\cite{graves2014neural} & copy, repeat copy, associative recall, Dynamic Ngrams, priority sort & input-output  \\
\addlinespace
\cite{balog2016deepcoder} & \parbox[t]{9.5cm}{DSL: 500 programs of length 3,4,5,generate 5 input-output examples per program, given the examples predict program using search} & input-output \\
\addlinespace
parisotto2016neuro & \parbox[t]{9.5cm}{DSL: randomly generate programs of length 13, generate 10 input-output strings for each program} & input-output \\
\addlinespace
\cite{bovsnjak2016programming} & sorting, addition, word algebra ($+, -, \times, \div$) &  \parbox[t]{2cm}{input-output + program sketch (not full program)}\\
\addlinespace
\cite{reed2015neural} & \parbox[t]{9.5cm}{learn 21 programs from image pixels categorized under: sort, addition, canonicalizing 3D models. 21 refers to subprograms such as shift that is needed in each category} & execution traces \\
\addlinespace
\cite{cai2017making} & bubble sort, topological sort, quicksort, grade-school addition & \parbox[t]{2cm}{execution traces of recursive programs} \\
\addlinespace
\cite{neelakantan2015neural} & \parbox[t]{9.5cm}{data: 50000 (question, table, answer) triplets. Arithmetic and logic operators such as greater than, less than, and, or. data is generated from a set of question templates such as: ``sum elements in column C''} & \parbox[t]{2cm}{input-output + program trace supervision} \\
\addlinespace
\cite{zaremba2014learning} & matrix/vector/scalar multiply, row/column sum, repeat, transpose & input-output \\
\addlinespace
\cite{allamanis2016learning} & $+,-,\times, \vee, \wedge, \neg, \implies, \oplus$ & symbolic data\\
\addlinespace
\cite{zaremba2016learning} & \parbox[t]{9.5cm}{this is Q-learning, not sure if we want to cite it. Copy, reverse, walk, addition, 3 digit addition}  & input-output \\
\addlinespace
\cite{loos2017deep} & \parbox[t]{9.5cm}{theorem proving: represents all functions/symbols,... in a dictionary and embeds their representation using a NN block} & \parbox[t]{2cm}{Mizar dataset of mathematical proofs} \\
\hline
\end{tabular}
\end{table}
}

\cut{
\begin{figure}
	\centering
        \begin{subfigure}{0.45\textwidth}
    	\includegraphics[width=\textwidth]{figs/inc_acc_both.pdf}
        \caption{Adding symbolic and function evaluation data}
        \label{fig:inc_acc_both}
        \end{subfigure}
        \begin{subfigure}{0.45\textwidth}

\includegraphics[width=\textwidth]{figs/inc_acc_sym_help_num_generalize.pdf}
%     	\includegraphics[width=\textwidth]{figs/inc_acc_sym_help_num_ave.pdf}
        \caption{Fixed symbolic data}
        \label{fig:inc_acc}
        \end{subfigure}
        \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{figs/inc_acc_sym_help_num_ave.pdf}
		\end{subfigure}
\label{fig:incAcc}
\caption{Accuracy per number of symbolic and function evaluation data added. In Fig (a) X axis label 1000 means that there were 1000 symbolic and 1000 function evaluation data in train. Test set is fixed and includes 8410 symbolic and function evaluation unseen expressions. Both train and test data include equations of depths [1,2,3,4]. Total number of symbolic and function evaluation equations at train are 14104 and 19523, respectively. Fig (b) is trained on equations of depth 1,3 and 4 and tested on function evaluations of depth 2. One curve has access to all the symbolic data, and Function evaluation data is added in the x axis. Fig (c) is trained on equations of depth [1,2,4] and tested on depth 3}
\end{figure}
        
\begin{figure}
	\centering
        \begin{subfigure}{0.45\textwidth}    	\includegraphics[width=\textwidth]{figs/inc_acc_num_train_num.pdf}
        \caption{Accuracy per number of function evaluation data on unseen numeric expressions}
        \label{fig:inc_acc_num}
        \end{subfigure}
        \begin{subfigure}{0.45\textwidth}
    	\includegraphics[width=\textwidth]{figs/inc_acc_sym_train_num.pdf}
        \caption{Accuracy per number of function evaluation data on unseen symbolic expressions}
        \label{fig:inc_acc_sym}
        \end{subfigure}
\label{fig:incAccData}
\caption{Accuracy per number of function evaluation data added. One curve is only trained on numeric data and one curve is trained on both numeric and symbolic data\sscomment{something feels missing. should there be sym-only for the latter?}}
\end{figure}


\begin{figure}
\centering
	\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/cos_prediction_noMask.pdf}
    \caption{Results of function evaluation for $\cos$}
    \label{fig:feval:cos}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/sin_prediction_noMask.pdf}
    \caption{Results of function evaluation for $\sin$}
    \label{fig:feval:sin}
    \end{subfigure}
    \caption{top-$1$ prediction for the identity completion task on two trigonometry functions.}
\end{figure}
%vertical green lines indicate if an identity was present in the training data or not. 1, means present and 0 means absent. Note: identities seen at train help the equation validation accuracy, but they do not necessary produce a top hit.

\begin{figure}
\centering
	\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/cos_prediction_train.pdf}
    \caption{Results of function evaluation for $\cos$ on train data}
    \label{fig:feval:cos:test_app}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/cos_prediction_test.pdf}
    \caption{Results of function evaluation for $\cos$ on test data}
    \label{fig:feval:cos:test}
    \end{subfigure}
    \caption{top-$1$ prediction for the identity completion task on two trigonometry functions.}
	\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/sin_prediction_train.pdf}
    \caption{Results of function evaluation for $\sin$}
    \label{fig:feval:sin:train}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/sin_prediction_test.pdf}
    \caption{Results of function evaluation for $\sin$ on test}
    \label{fig:feval:sin:test}
    \end{subfigure}
    \caption{top-$1$ prediction for the identity completion task on two trigonometry functions.}
\end{figure}
} 
